Electron-beam Calibration of Aerogel Tiles for the HELIX RICH Detector

The HELIX cosmic-ray detector is a balloon-borne instrument designed to measure the flux of light isotopes in the energy range from 0.2 GeV/n to beyond 3 GeV/n. It will rely on a ring-imaging Cherenkov (RICH) detector for particle identification at energies greater than 1 GeV/n and will use aerogel tiles with refractive index near 1.15 as the radiator. To achieve the performance goals of the experiment it is necessary to know the refractive index and its position dependence over the lateral extent of the tiles to a precision of O(10$^{-4}). In this paper we describe the apparatus and methods developed to calibrate the HELIX tiles in an electron beam, in order to meet this requirement.

==> geant4_section.tex <==

\section{Comparison with Monte-Carlo Simulations}

To further understand the electron beam data, the electron beam setup was simulated using \texttt{Geant4} (v11.0.1) \cite{AGOSTINELLI2003250, 1610988, ALLISON2016186}.
The simulation consisted of a mono-energetic beam, an aerogel tile with density and composition as described by \cite{tabata, tabata-2} and a shape matching a typical tile as measured using the CMM (see Section \ref{sec:radii}).
The \texttt{QGSP\_BIC\_HP\_EMZ} `physics list' was used with \texttt{G4OpticalPhysics} enabled. 

\par The CCD detector-board was simulated as a single plane with 100\% efficiency for detecting photons. 
The photon coordinates on hitting the board were recorded for later analysis.


\par To test for systematic shifts in the location of the maxima in the CCDs, with respect to the Cherenkov ring radius, simulations were conducted under two physical conditions. In the first, a `pencil beam' profile was used, with multiple Coulomb scattering, ionization losses, Compton and Rayleigh scattering, and bremsstrahlung processes disabled. This produces an idealized Cherenkov photon distribution, with a peak position at the Cherenkov ring radius. An example of this simulation is shown in Fig.~\ref{geant4_sim}. The width of the distribution is due to geometric aberration; Cherenkov photons originate at every point along the electron's passage through the aerogel tile. The width of this distribution is the product of the tangent of the Cherenkov angle and the thickness of the tile.

\par The second set of simulations was conducted with all physical processes enabled and a 2D Gaussian beam profile, where the profile parameters were chosen to match a typical beam profile measured during data acquisition. 
Beam divergence was included as a free parameter and varied to achieve the best agreement with the CCD distributions. 
The optimal value was found to be approximately $0.13^{\circ}$.
These simulations correspond to a `realistic beam' model.

\par The radial distance from the detector centre was calculated for each photon impact and recorded in a histogram with bin-width matching the CCD pixel size of 8 $\mu m$.
To mimic the analysis methods, these binned data were smoothed with a median filter with a kernel width of 9 entries.

\par The `pencil-beam' simulation resulted in a top-hat CCD distribution and its mean was used as the estimate of the Cherenkov ring radius. 
The corresponding parameter for the `realistic-beam' distributions was taken to be the maximum of the best-fit parabola to the photon distribution. 

\par The best-fit maximum, as shown in Fig.~\ref{geant4_sim}, shows a systematic shift between the `pencil beam' model and the `realistic beam' model. This shift is dominated by the effect of  multiple scattering. 

\par The simulations were repeated over refractive indices in the range [1.14,1.16] to confirm that these effects are independent of refractive index. 
The results are shown in Fig. \ref{geant4_shift}, where the peak shifts do not display any dependence on refractive index.


\par The shift means that a small systematic correction is required when calculating the refractive index
but it amounts to a single number for all the tiles.
This global correction will be measured using cosmic-ray muons during pre-flight tests of the integrated HELIX payload.


\begin{figure}
     \centering
     % \begin{subfigure}[b]{0.45\textwidth}
     %     \centering
     %     \includegraphics[width=1.1\textwidth]{figures/top-hat.pdf}
     %     \label{fig:top-hat}
     % \end{subfigure}
     % \hfill
     % \begin{subfigure}[b]{0.45\textwidth}
     %     \centering
     %     \includegraphics[width=1.1\textwidth]{figures/ste_parabola.pdf}
     %     \label{fig:parabola}
     % \end{subfigure}
     
        \vspace{0cm}
        \centerline{\includegraphics[width=1.\textwidth,angle=0.]{figures/PhotonPosition.png}}
        \vspace{0cm}
        \caption{Radial distributions of Cherenkov photons as simulated with Geant4.\\
        Left: a `pencil' beam with no divergence, and no scattering in the aerogel, produces a top-hat distribution, the result of geometric aberration due to the thickness of the tile.\\
        Right: with multiple scattering and a divergent beam, a parabolic distribution is produced and its maximum (red line) is displaced from the mean of the top-hat distribution (black line).}
        \label{geant4_sim}
\end{figure}




%\begin{figure}[h]
%\vspace{0cm}
%\centerline{\includegraphics[width=1.1\textwidth,angle=0.]{figures/Compare_n1.1575_35.png}}
%\vspace{0cm}
%\caption{Example of \texttt{Geant4} simulation result. The top panels show the results for a `pencil'-like beam with scattering and energy-loss processes (see text) turned off. The bottom panels show the results for a realistic beam model. The left panels show the 2D electron distribution at the location of the detector plane. The middle panel shows the electron energy distribution at the location of the detector plane. The right panel shows the photon distribution at the location of the detector plane. The black line shows the observed photon distribution with the orange line showing median-filtered data. The horizontal black and red lines show the mean location of the pencil-like photon distribution and the maximum of the parabola fit to the realistic photon distribution.
%}
%\label{geant4_sim}
%\end{figure}

\begin{figure}[h]
\vspace{0cm}
\centerline{\includegraphics[width=1.1\textwidth,angle=0.]{figures/ShiftInPeak.png}}
\vspace{0cm}
\caption{Differences of the kind shown in the right panel of Fig.~\ref{geant4_sim} plotted vs the refractive index used in the simulations. The solid and dashed black lines correspond to the mean and standard deviation of the measured points. See text for more details. 
}
\label{geant4_shift}
\end{figure}
